An SMT Based Compositional Algorithm to Solve a Conflict-Free Electric Vehicle Routing Problem

The Vehicle Routing Problem (VRP) is the combinatorial optimization problem of designing routes for vehicles to visit customers in such a fashion that a cost function, typically the number of vehicles, or the total travelled distance is minimized. The problem finds applications in industrial scenarios, for example where Automated Guided Vehicles run through the plant to deliver components from the warehouse. This specific problem, henceforth called the Electric Conflict-Free Vehicle Routing Problem (CF-EVRP), involves constraints such as limited operating range of the vehicles, time windows on the delivery to the customers, and limited capacity on the number of vehicles the road segments can accommodate at the same time. Such a complex system results in a large model that cannot easily be solved to optimality in reasonable time. We therefore developed a compositional model that breaks down the problem into smaller and simpler sub-problems and provides sub-optimal, feasible solutions to the original problem. The algorithm exploits the strengths of SMT solvers, which proved in our previous work to be an efficient approach to deal with scheduling problems. Compared to a monolithic model for the CF-EVRP, written in the SMT standard language and solved using a state-of-the-art SMT solver the compositional model was found to be significantly faster.

==> CASE_table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table*}[t]
  \centering
  \caption{Comparison of the compositional algorithm (CA) and the monolithic model (MM) for the \theModel ~over a set of generated problem instances. Instances are sorted by the parameters N-V-J (nodes, vehicles, jobs), value of edge reduction, and time horizon. For each resulting class, five instances are evaluated and the number of satisfied (sat) and unsatisfied (unsat) ones is reported, together with the average solving time (in seconds) for that specific class (ST-sat and ST-unsat respectively). If an instance is neither sat nor unsat then it is unknown. The average generation time (GT, in seconds) is also reported. The symbol ``-'' means that no instance for that category was either satisfiable or unsatisfiable, depending on where the symbol appears.}
  \resizebox{2\columnwidth}{!}{
    \begin{tabular}{cc|ccc|ccc|ccc|ccc|ccc|ccc}
    \toprule
       &    & \multicolumn{6}{c|}{15-3-5}  & \multicolumn{6}{c|}{25-4-6}  & \multicolumn{6}{c}{35-6-8} \\
       &    & \multicolumn{3}{c}{CA} & \multicolumn{3}{c|}{MM} & \multicolumn{3}{c}{CA} & \multicolumn{3}{c|}{MM} & \multicolumn{3}{c}{CA} & \multicolumn{3}{c}{MM} \\
    Time Horizon  &    & 0  & 25 & 50 & 0  & 25 & 50 & 0  & 25 & 50 & 0  & 25 & 50 & 0  & 25 & 50 & 0  & 25 & 50 \\
    \midrule
    \multirow{5}[2]{*}{15} & sat & 4  & 3  & 2  & 4  & 3  & 2  & 2  & 0  & 0  & 2  & 0  & 0  & 1  & 0  & 0  & 1  & 0  & 0 \\
       & unsat & 0  & 0  & 0  & 1  & 2  & 4  & 1  & 1  & 3  & 3  & 5  & 5  & 4  & 4  & 5  & 4  & 5  & 5 \\
       & GT & 1  & 1  & 0  & 23 & 23 & 22 & 1  & 1  & 1  & 75 & 68 & 70 & 2  & 2  & 1  & 167 & 132 & 132 \\
       & ST-sat & 4  & 5  & 14 & 11 & 9  & 11 & 14 & -  & -  & 42 & -  & -  & 12 & -  & -  & 80 & -  & - \\
       & ST-unsat & -  & -  & -  & 1  & 5  & 4  & 12 & 14 & 14 & 27 & 24 & 24 & 19 & 22 & 25 & 97 & 135 & 83 \\
    \midrule
    \multirow{5}[2]{*}{20} & sat & 4  & 3  & 3  & 4  & 3  & 3  & 5  & 4  & 1  & 5  & 4  & 1  & 4  & 4  & 4  & 4  & 4  & 4 \\
       & unsat & 0  & 0  & 0  & 1  & 2  & 2  & 0  & 0  & 1  & 0  & 1  & 4  & 1  & 1  & 1  & 1  & 1  & 1 \\
       & GT & 1  & 1  & 0  & 42 & 41 & 43 & 1  & 1  & 1  & 126 & 110 & 100 & 2  & 2  & 1  & 221 & 204 & 202 \\
       & ST-sat & 5  & 6  & 3  & 21 & 24 & 39 & 33 & 99 & 17 & 183 & 163 & 111 & 121 & 97 & 135 & 897 & 636 & 645 \\
       & ST-unsat & -  & -  & -  & 2  & 34 & 22 & -  & -  & 14 &    & 334 & 114 & 18 & 23 & 27 & 49 & 33 & 31 \\
    \midrule
    \multirow{5}[2]{*}{25} & sat & 4  & 3  & 3  & 5  & 3  & 3  & 5  & 4  & 1  & 5  & 4  & 2  & 4  & 4  & 4  & 4  & 4  & 4 \\
       & unsat & 0  & 0  & 0  & 0  & 1  & 1  & 0  & 0  & 1  & 0  & 0  & 1  & 1  & 1  & 1  & 1  & 1  & 1 \\
       & GT & 1  & 1  & 0  & 65 & 71 & 66 & 1  & 1  & 1  & 196 & 170 & 191 & 2  & 2  & 1  & 426 & 376 & 347 \\
       & ST-sat & 5  & 6  & 3  & 913 & 67 & 66 & 26 & 82 & 28 & 1161 & 995 & 480 & 96 & 84 & 46 & 2269 & 938 & 890 \\
       & ST-unsat & -  & -  & -  & -  & 845 & 5  & -  & -  & 14 & -  & -  & 1197 & 21 & 22 & 26 & 139 & 78 & 125 \\
    \midrule
    \multirow{5}[2]{*}{30} & sat & 4  & 3  & 3  & 5  & 3  & 3  & 5  & 4  & 1  & 4  & 4  & 2  & 4  & 4  & 4  & 4  & 4  & 4 \\
       & unsat & 0  & 0  & 0  & 0  & 0  & 1  & 0  & 0  & 1  & 0  & 0  & 0  & 1  & 1  & 1  & 0  & 1  & 1 \\
       & GT & 1  & 1  & 0  & 94 & 98 & 102 & 1  & 1  & 1  & 285 & 276 & 293 & 2  & 2  & 1  & 586 & 597 & 492 \\
       & ST-sat & 5  & 6  & 3  & 162 & 178 & 241 & 23 & 148 & 30 & 2312 & 3147 & 318 & 184 & 221 & 72 & 2689 & 1168 & 1262 \\
       & ST-unsat & -  & -  & -  & -  & -  & 902 & -  & -  & 14 & -  & -  & -  & 20 & 23 & 27 & -  & 914 & 210 \\
    \bottomrule
    \end{tabular}%

    }
  \label{tab:table_I}%
\end{table*}%


==> flow_chart.tex <==
\begin{algorithm}[H]
    \SetAlgoLined
    \LinesNumbered
    \SetKwInput{KwResult}{Output}
    \SetKwInput{kwData}{Input}
    \kwData{graph, jobs}
    \KwResult{instance, schedule}
    \caption{Compositional Algorithm}\label{decomp_algo}
        $\textrm{\textit{UsedPaths}} \gets []$ \\
        $PreviousRoutes \gets []$ \\
        $instance \gets unknown $ \\
        $PF \gets unknown $ \\
        $RF \gets unknown $ \\
        $AF \gets unknown $ \\
        $SF \gets unknown $ \\
        $Paths \gets path\_enumerator(graph,jobs) $ \\
        \While{$instance = unknown$}{
            $RF \gets unknown$ \\
            $PF,current\_path \gets path\_selection(Paths,\textrm{\textit{UsedPaths}})$ \\
            \eIf{$PF = unsat$}
                {$instance \gets PF$}
            {
                $UsedPaths \gets current\_path$ \\
                \While{$RF \neq unsat \wedge instance = unknown$}{
                    $RF,Routes \gets router(current\_path,PreviousRoutes) $ \\
                    \eIf{$RF = unsat$}
                        {\If{$PreviousRoutes = []$}
                            {$instance = unsat$}
                        { $PreviousRoutes \gets []$ }
                        }
                    {
                        $PreviousRoutes \gets Routes$ \\
                        $AF,assignment \gets assign(Routes)$ \\
                        \If{$AF = sat$}
                            {$SF,schedule \gets scheduler(assignment)$ \\
                            \If{$SF = sat$}
                                {$instance \gets SF$}
                            }
                            
                        
                        }
                    }
                }
        }
\end{algorithm}


==> reviewers__comments.tex <==
Associate Editor

I have completed my evaluation of your manuscript. The
reviewers recommend reconsideration of your manuscript
following major revision. I invite you to resubmit your
manuscript after addressing the comments below. 

Reviewer 777
The authors present an SMT based compositional model to
solve a conflict-free vehicle routing problem. 
The authors should make a clear description of the indexes
in the Table 1. eg: What does CA and S stands for? The
presentation of the experimental results is too
complicated. Not only the results should be satisfiable but
also optimized.

Reviewer 783
1.	How to avoid deadlock in the compositional model?
Are some instances unsatisfied due to deadlock?
2.	To improve readability, the essential grammar of
the SMT standard language applied in the compositional
model or the symbols/operators in the compositional model
should be explained or defined clearly in the first
occurrence.
3.	The experiment results in Table 1 show that the
number of the unsat instances for the compositional model
is equal to or larger than that for the monolithic model.
Does it mean that the monolithic model finds feasible
solutions for some instances but the compositional model
cannot find feasible solutions for these instances? The
authors state that ‘it is possible to notice that there is
a number of instances that were determined unknown by the
compositional model but were declared unsat by the
monolithic model’. How many instances are determined
unknown by the compositional model but are declared unsat
by the monolithic model?
4.	The illustrative example in Fig.1 and the instances
in Table 1 all use hypothetical data. How does the
compositional model perform using real industrial data?

